A deep study of open cluster NGC 5288 using photometric and astrometric data from Gaia DR3 and 2MASS

This paper investigates a poorly studied open cluster, NGC 5288, using 2MASS JHKS and the recently released Gaia DR3 astrometric and photometric data. The mean proper motions in Right Ascension and Declination are estimated as (-3.840 +/- 0.230) and (-1.934 +/- 0.162) mas/yr, respectively. We also derive the age and distance of the cluster as 510 +/- 190 Myr and 2.64 +/- 0.11 kpc, using colour-magnitude diagrams (CMDs). We have also obtained distance as 2.77 +/- 0.42 kpc using the parallax method. Interstellar reddening E(B-V) in the direction of the cluster is determined as 0.45 mag using the ((J - H), (J - K)) colour-colour diagram. We have found the mass function slope for main-sequence stars as 1.39 +/- 0.29 within the mass range 1.0 - 2.7 solar mass, which agrees with Salpeter's value within uncertainty. Galactic orbits are derived using the Galactic potential model, indicating that NGC 5288 follows a circular path around the Galactic center.

==> README <==
-------------------------
THE REVMEXAA LATEX MACROS
-------------------------

Version: 3.26b (09 Feb 2015)

Author: William Henney (w.henney@crya.unam.mx)

Latest version available from:	http://www.crya.unam.mx/rmaa


USAGE
-----

This package is intended for the typesetting of papers that are being
submitted for publication in the main journal of the Revista Mexicana
de Astronomia y Astrofisica. The example document
rm-journal-example.tex serves both as simple documentation and as a
template for your own contribution.

Further details on the use of the macros are given in the "Guide for
Authors", authorguide.pdf


VERSION 3.2x RELEASE NOTES 
--------------------------

The main change in this release is a reorganization to give separate
packages for the Conference Series (rmsc3.2x.tar.gz or rmsc3.2x.zip)
and the main journal (rmaa3.2x.tar.gz or rmaa3.2x.zip).

The manuscript option for the main journal has been revamped and this
is now the default style, which should be used for all submissions.

A maximum of six keywords is now enforced. Exceeding this limit gives
a LaTeX compilation error.

There is also support for BibTeX, and a "review article" option has
been added to the main journal.

For more details, see the News section of http://www.crya.unam.mx/rmaa

DOWNLOAD AND INSTALLATION
-------------------------

The latest version of the macros can always be obtained from
|http://www.astrosmo.unam.mx/rmaa|. There are three different
packages, each designed for a different audience: authors of main
journal papers (e.g., |rmaa3.24.tar.gz|), authors of contributions to
conference proceedings (e.g., |rmsc3.24.tar.gz|), and editors of the
main journal or conference proceedings (e.g.,
|rmaa_editor3.24.tar.gz|). Please make sure you have the right
package. All packages are also provided in |.zip| format, chiefly for
the convenience of MS Windows users.

Once you have downloaded the relevant package archive file, move it to
the directory (folder) where you wish to work and unpack the
archive. The procedure to do this may vary between systems. From the
command line on Unix, Linux, or Mac OS X, you can use something like
|tar -zxf rmaa3.24.tar.gz|.

To test that everything is working, you should compile the example
document: |rm-journal-example.tex|. You will need to invoke |latex|
twice to get the cross references right. The procedure to view and
print the document will vary between systems. On Unix, Linux, or Mac
OS X, you can use |latex} and |dvips| to generate a postscript file
(which can be converted to PDF via |ps2pdf|), or alternatively you can
use |pdflatex| to generate a PDF file directly. Note that in the first
case, any included graphics must be in EPS format, while in the second
case, they must be in PDF, PNG, or JPG format. It is recommended that
you omit the file extension from the filenames in the
|\includegraphics| command, so that both |latex| and |pdflatex| can
automatically find the correct figure file.

Assuming that the example document compiled and printed correctly, you
can now start writing your own paper, using the example document as a
template. 


FILE MANIFEST for rmaaN.MM.tar:
-------------------------------

README			this file
rmaa.cls		LaTeX class file for typesetting RMAA articles 
rm-journal-example.tex	Example main journal paper and tutorial
authorguide.pdf		Guide for Authors 
example-fig.eps		Example of figure
example-badfig.eps	Example of how not to do a figure
example-fig.pdf		
example-badfig.pdf	
rmaa.bst		Bibtex style file (experimental)
GPL			Terms and conditions for copying, distribution
                        and modification


